QLLM: Accurate and Efficient Low-Bitwidth Quantization for Large Language Models

Large Language Models (LLMs) excel in NLP, but their demands hinder their widespread deployment. While Quantization-Aware Training (QAT) offers a solution, its extensive training costs make Post-Training Quantization (PTQ) a more practical approach for LLMs. In existing studies, activation outliers in particular channels are identified as the bottleneck to PTQ accuracy. They propose to transform the magnitudes from activations to weights, which however offers limited alleviation or suffers from unstable gradients, resulting in a severe performance drop at low-bitwidth. In this paper, we propose QLLM, an accurate and efficient low-bitwidth PTQ method designed for LLMs. QLLM introduces an adaptive channel reassembly technique that reallocates the magnitude of outliers to other channels, thereby mitigating their impact on the quantization range. This is achieved by channel disassembly and channel assembly, which first breaks down the outlier channels into several sub-channels to ensure a more balanced distribution of activation magnitudes. Then similar channels are merged to maintain the original channel number for efficiency. Additionally, an adaptive strategy is designed to autonomously determine the optimal number of sub-channels for channel disassembly. To further compensate for the performance loss caused by quantization, we propose an efficient tuning method that only learns a small number of low-rank weights while freezing the pre-trained quantized model. After training, these low-rank parameters can be fused into the frozen weights without affecting inference. Extensive experiments on LLaMA-1 and LLaMA-2 show that QLLM can obtain accurate quantized models efficiently. For example, QLLM quantizes the 4-bit LLaMA-2-70B within 10 hours on a single A100-80G GPU, outperforming the previous state-of-the-art method by 7.89% on the average accuracy across five zero-shot tasks.

==> math_iclr.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

\def\ie{\mbox{\textit{i.e.}}}
\def\eg{\mbox{\textit{e.g.}}}


==> method_bak.tex <==
\subsection{Preliminary}
In this paper, we adopt uniform linear quantization
for both weights and activations
because of its hardware-friendly nature~\citep{jacob2018quantization}. Given a high-precision matrix $\bX$, \eg, half-precision (FP16) or full-precision (FP32), the $b$-bit quantization process can be defined as 
\begin{equation}
    \label{eq:quantization}
    \begin{split}
            \bX_q = \mathrm{quant}(\bX) = \mathrm{clamp} \left( \lfloor \frac{\bX}{\alpha} \rceil + \beta, 0, 2^b - 1 \right), ~\\
            \mathrm{where}~\alpha = \frac{\mathrm{max}(\bX) - \mathrm{min}(\bX) }{2^b - 1}, \beta = -\left\lfloor\frac{ \mathrm{min} (\mathbf{X})}{\alpha}\right\rceil,
    \end{split}
\end{equation}
where the function $\mathrm{clamp}(v, v_{\mathrm{min}}, v_{\mathrm{max}})$ clips any value $v$ into the range of $[v_{\mathrm{min}}, v_{\mathrm{max}}]$ and $\lfloor \cdot \rceil$ is a rounding operator that returns the nearest integer of a given value. Here, $\alpha$ denotes the scaling factor and $\beta$ represents the zero-point value.

\jing{Note that utilizing layer-wise quantization \bohan{for activations} is a common practice as it is hardware-friendly.} Given that the magnitude of outliers in activations is much larger than the other values, the quantization range determined by $\mathrm{min}(\bX)$ and $\mathrm{max}(\bX)$ in Eq.~(\ref{eq:quantization}) is inevitably skewed towards these extreme values. This means most values get squeezed into a narrow range during quantization, leading to a loss of information when they are converted to a few levels. Fortunately, recent research~\citep{dettmers2022gpt3,xiao2023smoothquant,wei2022outlier} has revealed that activation outliers appear in only a limited subset of channels. Based on this observation, it is often beneficial to employ a channel-wise quantization method, which uses distinct scaling factors and zero-points for different channels, resulting in much lower quantization error compared with %
layer-wise
quantization. However, the channel-wise activation quantization is not compatible with low-bitwidth general matrix multiplication (GEMM) kernels as it requires repeated rescalings in matrix multiplication~\citep{dettmers2022gpt3,bondarenko2021understanding}. \jing{As a result, prior studies~\citep{yao2022zeroquant,dettmers2022gpt3} have predominantly adopted token-wise quantization. While this method is GEMM-friendly, it nonetheless fails to adequately address the challenges associated with activation quantization.}



\subsection{Adaptive Channel Reassembly}
To address the above challenge, we propose a channel reassembly method that redistributes input activation outliers across multiple channels, which balances the distributions and consequently facilitates more accurate quantization. Our channel reassembly technique consists of three core components: channel disassembly, channel assembly, and an adaptive strategy. 
After channel reassembly, we further propose an efficient error correction to further improve the accuracy of quantized LLMs efficiently.

\subsubsection{Channel Disassembly}
\label{sec:CD}
\jing{Given a linear layer in LLMs, the goal of channel disassembly is to 
\bohan{decompose}
the input outlier channels into several sub-channels,}
aiming at reducing the outlier magnitude and making the activations more quantization-friendly without altering the layer output. Formally, considering a linear layer in LLMs, let $\bx \in \mathbb{R}^{{M}}$ be the input activations and $\by \in \mathbb{R}^{{N}}$ be the output for layer $l$. Here, ${M}$ and ${N}$ represent the input and output channel dimensions, respectively. Then, the linear layer output $\by_k$ with respect to $k$-th channel can be computed by
\begin{equation}
\label{eq:linear_function}
    \by_k = \sum_{i=1}^{{M}} \bx_i \bW_{ik}, 
\end{equation}
where $\bW \in \mathbb{R}^{{M} \times {N}}$ denotes the weight of the linear layer $l$. 
Before channel disassembly, we need to identify the outlier channels, which can be achieved by thresholding. Specifically, a channel is considered an outlier if the maximum activation value $\mathrm{max}(\bx_i)$ within the channel exceeds a threshold $\theta$. The methodology for determining the optimal value of $\theta$ will be discussed in Section~\ref{sec:adatpive}. Without loss of generality, we assume that only the last channel ${M}$ is identified as the outlier channel. This channel is then disassembled into $T = \lceil \mathrm{max}(\bx_{{M}}) / \theta \rceil$ sub-channels, each with a value divided by $T$ to maintain the equivalent output. As a result, we can rewrite Eq.~(\ref{eq:linear_function}) as:
\begin{equation}
    \label{eq:channel_disassembly}
    \by_k = \sum_{i=1}^{{M} - 1} \bx_i \bW_{ik} + \underbrace{\frac{\bx_{{M}}}{T} \bW_{M k} + \cdots + \frac{\bx_{{M}}}{T} \bW_{{M} k}}_{T ~\text{times}},
\end{equation}
where we introduce additional $T-1$ channels for both input and weight. \jing{While introducing more channels through disassembly does indeed make the quantization process more accommodating to variations in input, it also brings about additional computational costs. To solve this, channel assembly will be introduced in the subsequent section.}


\subsubsection{Channel Assembly} 
\label{sec:channel_assembly}
Note that the \jing{input} channel count increases to $M + T - 1$ after channel disassembly. \jing{Given the substantial quantity of channels in LLMs, it is possible to omit some unimportant channels or merge similar input channels to keep the original channel count $M$ for efficiency while maintaining outputs. To achieve this, a straightforward method is to use channel pruning~\citep{ma2023llm,sun2023simple} that removes the unimportant channels directly. However, this method may result in substantial information loss, especially when $T$ is large.} Motivated by recent studies~\citep{bolya2023token,bolya2023tokensd} that combine similar tokens, we propose a channel assembly method that delves into merging $T-1$ similar input channels by averaging their features. To accomplish this, the initial step is to define a metric for ``similar". 
Given channels $i$ and $j$, we can merge them by 
\begin{equation}
    \label{eq:channel_assembly}
    \bx_i \bW_{ik} + \bx_j \bW_{jk} \approx \frac{\bx_i + \bx_j}{2} \left(\bW_{ik} + \bW_{jk}\right),
\end{equation}
where $\frac{\bx_i + \bx_j}{2}$ and $\bW_{ik} + \bW_{jk}$ represent the merged activation and weight, respectively. 
With the aim of minimizing the information loss of channel assembly, we can define a distance metric $D(i,j)$ between channels $i$ and $j$ as
\begin{equation}
\begin{split}
    \label{eq:distance}
    D(i,j) &= \left\| \bx_i \bW_{ik} + \bx_j \bW_{jk} - \frac{\bx_i + \bx_j}{2} \left(\bW_{ik} + \bW_{jk}\right) \right\|_2^2 \\
    &= \left\| \frac{\bx_i \left( \bW_{ik} - \bW_{jk} \right)}{2} + \frac{\bx_j \left( \bW_{jk} - \bW_{ik} \right)}{2} \right\|_2^2,
\end{split}
\end{equation}
where $\left\| \cdot \right\|_2$ represents the $\ell_2$ norm. The above distance metric takes into account the difference in both \bohan{input} activation and weight between the two channels. 

With the channel distance defined, the next step is to determine which channels to aggregate efficiently, with the goal of reducing the total channel count by $T-1$. To address this, we propose using bipartite soft matching~\citep{bolya2023token,bolya2023tokensd} that first partitions the channels into two sets, each containing roughly equal sizes, and subsequently finds the $T-1$ most similar pairs between these two sets. For a detailed introduction of the bipartite soft matching, we refer the reader to Section~\ref{sec:bipartite_soft_matching} of the Appendix due to page limit. Notably, the channels disassembled from the outlier channels play a critical role in the performance of LLMs. Therefore, we do not assemble them. \jing{After the channel reassembly, which includes both disassembly and assembly, we acquire the reassembled input activations that are more amenable to quantization, along with the corresponding reassembled weights for layer $l$.}

\subsubsection{Adaptive Reassembly}
\label{sec:adatpive}
\bohan{In Section~\ref{sec:CD}, we use thresholding with a hyperparameter $\theta$ to identify outlier channels, which subsequently determines the channel count after channel disassembly. However, it is hard to choose $\theta$ in practice using human heuristics as distinct layers have different patterns of outliers, as shown in Figure \ref{fig:act_dist}. 
Furthermore, when dealing with an extreme outlier with a fixed threshold $\theta$, $T$ can become exceedingly large. This can lead to a substantial quantization error due to a distorted quantization range, along with an associated rise in channel merging error due to an increased merging ratio.
}
\begin{wrapfigure}{r}{0.5\textwidth}
  \vspace{-0.1in}
  \begin{center}
    \includegraphics[width=0.48\textwidth]{figures/act_min_max_dist_first_layer.pdf}
  \end{center}
  \vspace{-0.15in}
  \caption{An illustration of the maximum and minimum input activation values for the MSA and FFN layers in the first Attention-FFN block of LLaMA-1-65B.}
  \label{fig:act_dist}
\vspace{-0.25in}
\end{wrapfigure}
To address this, motivated by~\citep{wei2023outlier}, \jing{we propose an adaptive strategy to find the optimal $\theta$ by minimizing the reassembly error between the original output activations and their counterparts generated with the reassembled input activations \bohan{for each layer}.}

Note that our channel reassembly technique can yield the reassembled activation $\hat{\bX} \in \mathbb{R}^{L \times M}$ with a sequence length of $L$, which can then be fed into a Multi-head Self-Attention (MSA) layer or a Feed-Forward Network (FFN) layer.
For example, let us consider a case where $\hat{\bX}$ is fed into a MSA layer. A standard MSA layer calculates queries, keys and values with three learnable projection matrices $\bW_Q, \bW_K, \bW_V \in \mathbb{R}^{M \times N}$ as $\bQ = \bX \bW_Q, \bK = \bX \bW_K, \bV = \bX \bW_V$, where $\bX \in \mathbb{R}^{L \times M}$ represents the original input activation. Let $\hat{\bW}_Q$, $\hat{\bW}_K$, $\hat{\bW}_V$ be the reassembled projection weights. 
In this way, the reconstructed queries, keys, and values can be formulated as
\begin{equation}
    \hat{\bQ} = \mathrm{quant}(\hat{\bX}) \mathrm{quant}(\hat{\bW_Q}), \hat{\bK} = \mathrm{quant}(\hat{\bX})\mathrm{quant}(\hat{\bW_K}), \hat{\bV} = \mathrm{quant}(\hat{\bX}) \mathrm{quant}(\hat{\bW_V}).
\end{equation}
We then find $\theta$ by solving the following problem
\begin{equation}
    \label{eq:problem_attn_mse}
    \arg\min_{\theta} \left \| \mathrm{Softmax}( \bQ\bK^{\top} ) \bV - \mathrm{Softmax}( \hat{\bQ} \hat{\bK}^{\top}) \hat{\bV} \right \|_F^2,
\end{equation}
where $\left \| \cdot \right \|_F$ denotes the Frobenius norm. To solve problem~(\ref{eq:problem_attn_mse}) efficiently, we use grid search following~\citep{choukroun2019low,wei2023outlier}.
\bohan{We summarize the proposed adaptive channel reassembly in Algorithm~\ref{alg:adaptive_channel_reassembly}.}

\subsubsection{Efficient implementation for channel reassembly}
\label{sec:efficient_reassembly}
Both channel disassembly and assembly can be implemented efficiently if the previous layer $l - 1$ is a linear layer. For channel disassembly, this involves enlarging the output weight channels of the preceding linear layer $l-1$ and the input weight channels of the current layer $l$ with appropriate scaling in an offline manner.
Similarly, channel assembly can be implemented by reducing the output weight channels of the preceding linear layer $l-1$ and adjusting
the input weight channels of the current layer $l$ with appropriate scaling. In cases where the preceding layer $l - 1$ is a non-linear layer, such as a layer normalization~\citep{ba2016layer}, we introduce additional disassembly and assembly layers that are designed to decompose and aggregate channels during runtime, with the channel 
indexes
for decomposition and aggregation calculated offline using calibration data, which only introduces a minor extra overhead.
More details can be found in Appendix. An empirical study for the inference time can be found in Section~\ref{sec:ablation_study}.

\subsection{Efficient error correction} 
\label{sec:efficient_error_correction}
After performing channel reassembly for all layers, we further propose an efficient error correction to improve the performance of the quantized LLMs \jing{using a small set of calibration data}. 
Inspired by recent developments in parameter-efficient fine-tuning methods~\citep{hu2022lora,dettmers2023qlora}, our efficient error correction introduces two low-rank parameters $\bA \in \mathbb{R}^{M \times r}$ and $\bB \in \mathbb{R}^{r \times N}$ with a rank of $r$ into each projection layer of our QLLM. 
Then, we can obtain the output $\bY$ of a quantized linear layer by
\begin{equation}
    \bY = \mathrm{quant}(\bX) \mathrm{quant}(\bW) + \mathrm{quant}(\bX) \bA \bB.
\end{equation}
\bohan{Instead of directly tuning the quantized weights, we learn the introduced low-rank parameters by minimizing the reconstruction error between the original and the quantized outputs of the Attention-FFN block. Thanks to the reduced number of trainable parameters, both the optimization cost and GPU memory usage can be significantly reduced. 
Such efficiency gain allows us to further 
suppress the accumulation of quantization error during forward propagation via a structured reconstruction, \ie, performing multi-block reconstruction for QLLM, which simultaneously adjusts a collection of consecutive Attention-FFN blocks by focusing on reconstructing the final block output.}




After the reconstruction, we only need to store the quantized weight $\mathrm{quant}(\bW + \bA\bB)$, which does not introduce extra inference cost.
However, it is inevitable that the absorption process will introduce additional quantization error. To counteract this, following~\citep{he2017channel,nagel2020up,hubara2020improving}, we perform reconstruction sequentially rather than in parallel, which enables us to account for the quantization error stemming from the previous layers.





